A Track-Before-Detect Algorithm for UWB Radar Sensor Networks

Precise localization and tracking of moving non-collaborative persons and objects using a network of ultra-wideband (UWB) radar nodes has been shown to represent a practical and effective approach. In UWB radar sensor networks (RSNs), existence of strong clutter, weak target echoes, and closely spaced targets are obstacles to achieving a satisfactory tracking performance. Using a track-before-detect (TBD) approach, the waveform obtained by each node during a time period are jointly processed. Both spatial information and temporal relationship between measurements are exploited in generating all possible candidate trajectories and only the best trajectories are selected as the outcome. The effectiveness of the developed TBD technique for UWB RSNs is confirmed by numerical simulations and by two experimental results, both carried out with actual UWB signals. In the first experiment, a human target is tracked by a monostatic radar network with an average localization error of 41.9 cm with no false alarm trajectory in a cluttered outdoor environment. In the second experiment, two targets are detected by multistatic radar network with localization errors of 25.4 cm and 19.7 cm, and detection rate of the two targets is 88.75%, and no false alarm trajectory.

==> code_design.tex <==
\begin{newcontentrevone}
\section{Code Design Examples} \label{sec:code_design}
In this section we provide several code design examples that illustrate the practical impact of the derived bounds.



\subsection{Design of a Binary Raptor code with an LDPC Outer Code}\label{sec:code_design:inner}



We consider the case in which the outer code ensemble is given and run a computer search in order to find an LT output degree distribution that optimizes a given metric subject to some design constraints. 
%
In particular, we consider Raptor code ensembles where the outer code is picked from the $(d_v=3, d_c=33)$ binary regular LDPC ensemble with $k=1000$  and $h=1100$, and we set as requirement 
minimizing the inactivation decoding complexity subject to a decoding failure probability not exceeding $10^{-3}$.

%
Inactivation decoding \cite{shokrollahi2005systems} is the efficient \ac{ML} decoding algorithm %, which is 
used to decode standardized Raptor codes \cite{MBMS16:raptor,luby2007rfc}.
%
%Inactivation decoding %
It can be seen as an extension of iterative (peeling) decoding where, whenever the iterative decoding process stops, an input symbol is declared as inactive, so that iterative decoding is resumed. At the end, one is left with a number of input symbols that have been inactivated, and whose values have to be recovered by means of Gaussian elimination. 
After doing so, all input symbols can be resolved  by back-substitution (i.e., using iterative decoding).
%
The complexity of inactivation decoding is generally dominated by the Gaussian elimination step, whose complexity is cubic on the number of inactivations. 
Thus, 
the number of inactivations can be used as a proxy to decoding complexity,
%. In other words, decoding complexity 
which is minimized by minimizing it. %the number of inactivations.
%

The degree distribution $\Omegarten$, given in \eqref{eq:dist_mbms}, has been designed for inactivation decoding. However, as it can be observed in Fig.~\ref{fig:LDPC_Design}, if we use $\Omegarten$  we do not fulfill the probability of failure constraint, since there is an error floor around $2 \times 10^{-3}$. Thus, we need carry out an ad-hoc design.

The analysis presented in \cite{lazaro2017inactivation} can be used to determine the expected number of inactivations for LT codes. Extending the analysis to Raptor codes is not easy, but, as it was shown in \cite{lazaro2017inactivation}, when the parity-check matrix of the outer code is considerably denser than the generator matrix of the inner LT code, it is possible to design Raptor codes that require few inactivations by optimizing the LT output degree distribution in isolation. In other words, if we design an LT degree distribution that requires few inactivations, and then construct a Raptor code using this degree distribution for the inner LT code,  we obtain a Raptor code that requires few inactivations.

Following this approach, we can use simulated annealing \cite{kirkpatrick1983optimization} to design an LT degree distribution that minimizes the number of inactivations under the constraint on the decoding failure probability, estimated by using the upper bound.
%
By using this approach we obtained the following degree distribution
\begin{align}
    \Omega_{\mathsf{B}} & = 0.0108 \x + 0.4557 \x^2  +  0.1959 \x^3   + 0.1195 \x^4   + 0.0245 \x^5  +0.0243 \x^6 
    + 0.0357  \x^{10} \\
    & \phantom{=}+  0.0412 \x^{11} + 0.0440 \x^{15} + 0.0196 \x^{21} + 0.0115 \x^{26} 
    + 0.0088 \x^{30} + 0.0085 \x^{40}. \label{deg_dist_ldpc}
\end{align}

\begin{figure}
    \centering
    \includegraphics[width=10cm]{./figures/LDPC_design}
    \caption{\revone{Average probability of decoding failure $\barPf$ vs absolute overhead for 4 different Raptor code ensembles.  
    The first and second ensemble have outer codes randomly drawn from the binary $(d_v=3, d_c= 33)$ regular LDPC ensemble  with $k=1000$ input symbols. For the second and third ensembles the outer codes are randomly drawn from the $(d_v=3, d_c= 63)$ regular LDPC ensemble  with $k=200$ and the $(d_v=3, d_c= 15)$ regular LDPC ensemble  with $k=100$. 
    The LT degree distributions are $\Omega_{\mathsf{A}}$, $\Omega_{\mathsf{B}}$, $\Omega_{\mathsf{C}}$ and $\Omega_{\mathsf{D}}$, respectively.
    Lines: upper bounds. Markers: simulation results.}}\label{fig:LDPC_Design}
\end{figure}

Fig.~\ref{fig:LDPC_Design} shows the average probability of decoding failure and its upper bound in Corollary~\ref{corollary:rateless} for the designed ensemble based on $\Omega_{\mathsf{B}}$.  We can observe how the Raptor code ensemble meets the design requirement, since $\barPf < 10^{-3}$ for $\absoverhead=15$. 

If we now consider the number of inactivations, we have that the designed Raptor code ensemble, which employs $\Omega_{\mathsf{B}}$,  needs in average $94$ inactivations for an absolute overhead $\absoverhead=15$. In constrast, the Raptor code ensemble employing $\Omegarten$ needs $87$.
%
This confirms how a reduction in the number of inactivations forces the failure rate to jump above the maximum tolerable value. 


\subsection{Design of a Nonbinary Raptor code with an LDPC Outer Code}\label{sec:code_design:nonbinary}

This design example is similar to the previous one, but this time we focus on a nonbinary Raptor code ensemble. In particular we aim at designing a Raptor code ensemble over $\GF4$, where the outer code is taken from the  $(d_v=3, d_c=63)$ regular LDPC ensemble with $k=200$  and $h=210$. The goal is minimizing the number of inactivations\footnote{The analysis in \cite{lazaro2017inactivation} is also valid for non-binary codes. The number of inactivations is a product of the first phase of inactivation decoding, triangulation, which is equivalent to column and row swapping and does not carry out any operations over the finite field. Thus, the number of inactivations only depends on the elements of the generator matrix of the LT code being zero or nonzero, and not on the particular value in  $\GF{q} \setminus \{0\}$ that the elements take.} subject to $\barPf \leq 10^{-4}$ at $\delta=10$. Using simulated annealing, the following degree distribution is obtained:
\begin{align}
    \Omega_{\mathsf{C}}(\x) & = 0.0214 \x + 0.3213 \x^2  +  0.2971 \x^3   + 0.0276 \x^4   + 0.0252 \x^5  +0.0418 \x^9 
    + 0.0458  \x^{13} \\
    & \phantom{=}+  0.0654 \x^{18} + 0.0457 \x^{23} + 0.0612 \x^{30} + 0.0295 \x^{35} 
    + 0.0180 \x^{40}. \label{deg_dist_nonbinary}
\end{align}
%
Fig.~\ref{fig:LDPC_Design} shows the average probability of decoding failure for the  ensemble obtained from the code design. We can observe how the constraint on $\barPf$ is fulfilled. The average number of inactivation needed for decoding at $\absoverhead=10$ is approximately $32$.

\subsection{Design of a Raptor Code with a  $0/1$ LT Code}\label{sec:code_design_met_etc}

We now address the design of a nonbinary Raptor code ensemble with a $0/1$ LT code. We aim at designing a Raptor code ensemble over $\GF4$, where the outer code is taken from the  $(d_v=3, d_c=15)$ regular LDPC ensemble with $k=100$  and $h=125$. The goal is minimizing the number of inactivations subject to $\barPf \leq 2 \times 10^{-3}$ at $\delta=5$. Using simulated annealing, the following degree distribution is obtained:
\begin{align}
    \Omega_{\mathsf{D}}(\x) & = 0.0095 \x + 0.3896 \x^2  +  0.3159 \x^3   + 0.0843 \x^4   + 0.0611 \x^{10}  +0.0585 \x^{15} + 0.0811  \x^{22}. \label{deg_dist_01}
\end{align}
%
Fig.~\ref{fig:LDPC_Design} shows the average probability of decoding failure for the designed ensemble. We can observe how the constraint on $\barPf$ is fulfilled. The average number of inactivations needed for decoding at $\absoverhead=5$ is approximately $22$.


\end{newcontentrevone}

==> reference.tex <==
\cite{win2011network}
\cite{withington2003enhancing}
\cite{bartoletti2014sensor}
\cite{chiani2018sensor}
\cite{giorgetti2016robust}
\cite{giorgetti2013time}
\cite{pinto2009stochastic}
\cite{paolini2008localization}
\cite{errasti2014track}
\cite{kwon2019particle}
\cite{ubeda2017adaptive}
\cite{yan2017track}
\cite{wei2010tbd}
\cite{yi2013efficient}
\cite{yan2019three}
\cite{yan2019detection}
\cite{moyer2011multi}
\cite{yan2019grey}
\cite{grossi2013heuristic}
\cite{wang2018greedy}
\cite{you2016radar}
\cite{chen2012modern}
\cite{levanon1990order}
\cite{rohling1983radar}
\cite{gao2017cfar}
\cite{yan2018efficient}
\cite{yan2017improved}
\cite{granstrom2012extended}
\cite{granstrom2015gamma}
\cite{lundquist2013extended}
\cite{yan2019improved}
\cite{yan2019efficient}
\cite{li2005survey}
\cite{punithakumar2008multiple}
\cite{hong2009novel}
\cite{yan2018improved}
\cite{musicki2004joint}
\cite{blom2015jipda}
\cite{chen2013integrated}
\cite{koch1997multiple}
\cite{palkki2011addressing}
\cite{wong2014bernoulli}
\cite{wan2003symmetric}
\cite{li20193d}
\cite{maintz20013d}
\cite{grinzato1998corrosion}
\cite{bieniek2000efficient}
\cite{mangan1999partitioning}
\cite{sahoo1998mean}
\cite{chong2000architectures}
\cite{blackman2004multiple}
\cite{ristic2010performance}

